Understanding the Context of IoT Software Systems in DevOps

The growing demand for connected devices and the increase in investments in the Internet of Things (IoT) sector induce the growth of the market for this technology. IoT permeates all areas of life of an individual, from smartwatches to entire home assistants and solutions in different areas. The IoT concept is gradually increasing all over the globe. IoT projects induce an articulation of studies in software engineering to prepare the development and operation of software systems materialized in physical objects and structures interconnected with embedded software and hosted in clouds. IoT projects have boundaries between development and operation stages. This study search for evidence in scientific literature to support these boundaries through Development and Operations (DevOps) principles. We rely on a Systematic Literature Review to investigate the relations of DevOps in IoT software systems. As a result, we identify concepts, characterize the benefits and challenges in the context of knowledge previously reported in primary studies in the literature. The main contributions of this paper are: (i) discussion of benefits and challenges for DevOps in IoT software systems, (ii) identification of tools, concepts, and programming languages used, and, (iii) perceived pipeline for this kind of software development.

==> tables/Studies.tex <==
\begin{table*}[!h]
\center
\caption{List of studies selected}\label{tab:tab2}
\begin{tabular}{lp{14cm}l}
\toprule
\small{Reference} & \small{Title} & \small{Venue type}\\
\midrule
\small{\cite{s01}} & \small{Dyn Tail - Dynamically Tailored Deployment Engines for Cloud Applications} & \small{Conference}\\
\small{\cite{s02}} & \small{DevOps for IoT Applications using Cellular Networks and Cloud} & \small{Conference}\\
\small{\cite{s03}} & \small{Automated Deployment of SmartX IoT-Cloud Services based on Continuous Integration} & \small{Conference}\\
\small{\cite{s04}} & \small{Application Development and Deployment for IoT Devices} & \small{Conference}\\
\small{\cite{s05}} & \small{A framework for evaluating continuous microservice delivery strategies} & \small{Conference}\\
\small{\cite{s06}} & \small{Verification and Validation Framework for 5G Network Services and Apps} & \small{Conference}\\
\small{\cite{s07}} & \small{Deployment Specification Challenges in the Context of Large Scale Systems} & \small{Conference}\\
\small{\cite{s08}} & \small{Architecting Enterprise Applications for the Cloud: The Unicorn Universe Cloud Framework} & \small{Workshop}\\
\small{\cite{s09}} & \small{A Roadmap to the Programmable World: Software Challenges in the IoT Era} & \small{Magazine}\\
\small{\cite{s10}} & \small{A manifesto for future generation cloud computing: Research directions for the next decade} & \small{Journal}\\
\small{\cite{s11}} & \small{Microservice-Based Agile Architectures: An Opportunity for Specialized Niche Technologies} & \small{Conference}\\
\small{\cite{s12}} & \small{A Microservice Architecture for the Industrial Internet-Of-Things} & \small{Conference}\\
\small{\cite{s13}} & \small{ENACT: Development, Operation, and Quality Assurance of Trustworthy Smart IoT Systems} & \small{Workshop}\\
\small{\cite{s14}} & \small{A reference architecture for the container ecosystem} & \small{Conference}\\
\small{\cite{s15}} & \small{DevOps Reference Architecture for Multi-Cloud IOT Applications} & \small{Conference}\\
\small{\cite{s16}} & \small{The Next Generation Platform as a Service Cloudifying Service Deployments in Telco-Operators Infrastructure} & \small{Conference}\\
\small{\cite{s17}} & \small{Towards a Model-Based DevOps for Cyber-Physical Systems} & \small{Workshop}\\
\small{\cite{s18}} & \small{Development and Operation of Trustworthy Smart IoT Systems: The ENACT Framework} & \small{Workshop}\\
\small{\cite{s19}} & \small{Self-Service Cybersecurity Monitoring as Enabler for DevSecOps} & \small{Magazine}\\
\small{\cite{s20}} & \small{RADON: rational decomposition and orchestration for serverless computing} & \small{Journal}\\
\small{\cite{s21}} & \small{On Observability and Monitoring of Distributed Systems: An Industry Interview Study} & \small{Conference}\\
\small{\cite{s22}} & \small{Towards Model-Based Continuous Deployment of Secure IoT Systems} & \small{Conference}\\
\small{\cite{s23}} & \small{A Survey of DevOps Concepts and Challenges} & \small{Journal}\\
\small{\cite{s24}} & \small{iIoT Ecosystem Development through Boundary Resources: A Siemens MindSphere Case Study} & \small{Workshop}\\
\small{\cite{s25}} & \small{The evolution of the Internet of Things (IoT): A computational text analysis} & \small{Journal}\\
\small{\cite{s26}} & \small{CloudsStorm: A framework for seamlessly programming and controlling virtual infrastructure functions during the DevOps lifecycle ofcloud applications} & \small{Journal}\\
\bottomrule
\end{tabular}
\end{table*}
